Function-constrained Program Synthesis

This work introduces (1) a technique that allows large language models (LLMs) to leverage user-provided code when solving programming tasks and (2) a method to iteratively generate modular sub-functions that can aid future code generation attempts when the initial code generated by the LLM is inadequate. Generating computer programs in general-purpose programming languages like Python poses a challenge for LLMs when instructed to use code provided in the prompt. Code-specific LLMs (e.g., GitHub Copilot, CodeLlama2) can generate code completions in real-time by drawing on all code available in a development environment. However, restricting code-specific LLMs to use only in-context code is not straightforward, as the model is not explicitly instructed to use the user-provided code and users cannot highlight precisely which snippets of code the model should incorporate into its context. Moreover, current systems lack effective recovery methods, forcing users to iteratively re-prompt the model with modified prompts until a sufficient solution is reached. Our method differs from traditional LLM-powered code-generation by constraining code-generation to an explicit function set and enabling recovery from failed attempts through automatically generated sub-functions. When the LLM cannot produce working code, we generate modular sub-functions to aid subsequent attempts at generating functional code. A by-product of our method is a library of reusable sub-functions that can solve related tasks, imitating a software team where efficiency scales with experience. We also introduce a new "half-shot" evaluation paradigm that provides tighter estimates of LLMs' coding abilities compared to traditional zero-shot evaluation. Our proposed evaluation method encourages models to output solutions in a structured format, decreasing syntax errors that can be mistaken for poor coding ability.

==> Figs/Results/ablations.tex <==

\begin{figure}[!t]
    \centering
    
    \begin{minipage}{0.43\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figs/Results/splits_plot.png}
       
    \end{minipage}
    \hfill
    \begin{minipage}{0.43\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figs/Results/num_skills_mod.png}
    \end{minipage}
    \caption{(right) Impact of \(|V^*|\) on Performance in \(HE_{CF}\); (left) Analyzing Accuracy on the \(HE_{BP,R}\) Dataset Relative to the Size of the Constraint}
    \label{fig:ablations}
\end{figure}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width = 0.6\textwidth]{Figs/Results/num_skills_plot_mod.png}
%     \caption{\textbf{Impact of $\mathbf{|V^*|}$ on Performance in $\mathbf{HE_{CF}}$}.
%     % This figure analyzes the relationship between the number of functions included in $V^*$ and performance on the $HE_{CF}$ dataset, using functions proposed by GPT-4 (blue), GPT-3.5 (orange), and a human expert (red). The details of the proposed functions are provided in Figures \ref{fig:all_skills_table}. The batch of functions marked in purple are the perfect-handwritten skills after being refined by GPT-4. Results for sub-skills proposed by a non-expert human (Adnaan) are presented in green. The black dot on the right bar plot represents the naive expected accuracy when all functions are added ($|V^*| = 8$), matching the average accuracy across all 8 questions when only a single function is included in the constrained model's context when solving the related question. The model is only able to achieve 50\% of its one-at-a-time accuracy when all human-written functions are provided (red bar plot). But when providing all functions generated by GPT-4, the model achieves 120\% of its one-at-a-time accuracy (blue bar plot).
%     }
%     \label{fig:numskills_plot}
% \end{figure}
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width = 0.6\textwidth]{Figs/Results/splits_plot.png}
%    \caption{{Analyzing Accuracy on the $HE_{BP,R}$ Dataset Relative to the Size of the Constraint.}
%    % We evaluate the accuracy of GPT-3.5 on the $HE_{BP,R}$ dataset with different amounts of replicas enforced. The percentage of replicas enforced is determined by the number of occurrences corresponding to the functions within the current subset of replicas $V_{sub}$. There are many ways to split the replicas into roughly even groups of four. Each ``split'' is a unique way. Detailed information about these splits can be found in Sec. \ref{sec:splits_expsetup}. Critically, when a function from $V_{rep}$ is not included in the enforced replicas, its Python Standard Library equivalent is not considered an invalid function. The most noticeable drop in performance occurs with the initial constraint of only a few replicas, suggesting that imposing a constraint, even a minor one, is what significantly impacts the model's performance. In certain scenarios, performance starts to rise as more functions are included, possibly due to the model learning from the code supplied for new replicas. When all replicas are enforced (100\% on the x-axis), different accuracies are observed for different splits, creating a variability of about +/- 5\% in accuracy. This variation stems from the fact that, for each split, the ordering of replicas in the prompt is different.
%    }
%     \label{fig:split_results}
% \end{figure}

==> Figs/Results/acc_v_replications.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width = 0.6\textwidth]{Figs/Results/splits_plot.png}
   \caption{{Analyzing Accuracy on the $HE_{BP,R}$ Dataset Relative to the Size of the Constraint.}
   % We evaluate the accuracy of GPT-3.5 on the $HE_{BP,R}$ dataset with different amounts of replicas enforced. The percentage of replicas enforced is determined by the number of occurrences corresponding to the functions within the current subset of replicas $V_{sub}$. There are many ways to split the replicas into roughly even groups of four. Each ``split'' is a unique way. Detailed information about these splits can be found in Sec. \ref{sec:splits_expsetup}. Critically, when a function from $V_{rep}$ is not included in the enforced replicas, its Python Standard Library equivalent is not considered an invalid function. The most noticeable drop in performance occurs with the initial constraint of only a few replicas, suggesting that imposing a constraint, even a minor one, is what significantly impacts the model's performance. In certain scenarios, performance starts to rise as more functions are included, possibly due to the model learning from the code supplied for new replicas. When all replicas are enforced (100\% on the x-axis), different accuracies are observed for different splits, creating a variability of about +/- 5\% in accuracy. This variation stems from the fact that, for each split, the ordering of replicas in the prompt is different.
   }
    \label{fig:split_results}
\end{figure}

==> Figs/Results/all_figs_combined.tex <==
\begin{figure}[t]
    \centering
    
    % Top-left and top-right figures
    \begin{minipage}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=6cm]{Figs/Results/utilisation_rate.png}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=6cm]{Figs/Results/non_compliance_rate.png}
    \end{minipage}
    
    \vspace{0.1mm} % Adjust this to control the vertical space between the two rows of images
    
    % Bottom-left and bottom-right figures
    \begin{minipage}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=6cm]{Figs/Results/splits_plot.png}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=6cm]{Figs/Results/num_skills_mod.png}
    \end{minipage}
    
    \caption{Top-left: GPT-4 is only evaluated on the top-three prompt configurations to reduce cost. Top-right: [Your description for the second image in the first figure here]. Bottom-left: Analyzing Accuracy on the \(HE_{BP,R}\) Dataset Relative to the Size of the Constraint. Bottom-right: Impact of \(|V^*|\) on Performance in \(HE_{CF}\).}
    \label{fig:combined_fig}
\end{figure}

==> Figs/Results/all_tables.tex <==

\begin{figure}[!htb]
    \centering
    % First table
    \begin{minipage}{1\textwidth}
        \centering
       \begin{tabular}{lllllllll|ll}
\toprule
\textbf{} & \textbf{2} & \textbf{84} & \textbf{89} & \textbf{79} & \textbf{154} & \textbf{110} & \textbf{65} & \textbf{82} & \textbf{PU} & \textbf{GU} \\
\midrule
\textbf{get\_decimal\_part}          &  Pass &   F &     F &     F &     F &     F &     F &   F &   1  &  0   \\
\textbf{sum\_of\_digits}             &     F &   F &     F &     F &     F &     F &     F &   F & 0    &  0   \\
\textbf{join\_list\_to\_string}       &     F &   F &     F &     F &  Pass &     F &     F &   F &  0   &   0.12  \\
\textbf{format\_binary\_string}      &     F &   F &     F &  Pass &  Pass &     F &     F &   F &    1 & 0.25    \\
\textbf{rotate\_string}             &     F &   F &  Pass &     F &  Pass &     F &     F &   F &  1   &  0.25   \\
\textbf{count\_even\_numbers}        &     F &   F &     F &     F &  Pass &  Pass &     F &   F &  1   &   0.25  \\
\textbf{calculate\_effective\_shift} &  Pass &   F &     F &     F &     F &     F &  Pass &   F &  1   &  0.25   \\
\textbf{is\_divisible}              &     F &   F &     F &     F &     F &     F &     F &   F &  0   &  0   \\
\bottomrule
\end{tabular}
    \end{minipage}
    \vspace{1em} % Space between tables

    % Third table (You can copy one of the above tables as a placeholder and modify it)
    \begin{minipage}{1\textwidth}
        \centering
        \begin{tabular}{lllllllll|ll}
\hline
\textbf{} & \textbf{2} & \textbf{84} & \textbf{89} & \textbf{79} & \textbf{154} & \textbf{110} & \textbf{65} & \textbf{82} & \textbf{PU} & \textbf{GU} \\
\hline
\textbf{get\_decimal\_part}     &  Pass &   F &     F &   F &  Pass &     F &     F &     F &    1  &   0.25   \\
\textbf{sum\_of\_digits\_binary} &  Pass &   F &     F &   F &  Pass &  Pass &     F &  Pass &  0    &    0.50  \\
\textbf{shift\_character}      &     F &   F &  Pass &   F &  Pass &     F &  Pass &     F &   1   &   0.37   \\
\textbf{add\_extra\_characters} &     F &   F &     F &   F &  Pass &     F &     F &     F &    0  &  0.12    \\
\textbf{is\_rotation}          &     F &   F &     F &   F &     F &     F &     F &     F &   0   &   0   \\
\textbf{count\_even\_elements}  &     F &   F &  Pass &   F &  Pass &  Pass &     F &     F &  1    &  0.37    \\
\textbf{reverse\_string}       &     F &   F &     F &   F &     F &     F &  Pass &     F &   1   &   0.12   \\
\textbf{is\_prime}             &     F &   F &     F &   F &  Pass &     F &     F &  Pass &  1    &   0.25   \\
\hline
\end{tabular}

    \end{minipage}
    \vspace{1em} % Space between tables

    % Second table
    \begin{minipage}{1\textwidth}
        \centering
        \begin{tabular}{lllllllll|lll}
\toprule
\textbf{} & \textbf{79} & \textbf{154} & \textbf{89} & \textbf{82} & \textbf{110} & \textbf{84} & \textbf{65} & \textbf{2} & \textbf{PU} & \textbf{GU} \\
\midrule
\textbf{remove\_bin\_prefix}       &  Pass &   F &     F &     F &     F &     F &     F &   F &  1   &  0.12   \\
\textbf{rotate\_string}             &     F &   Pass &     F &     F &     F &     F &     F &   F &   1  &  0.12   \\
\textbf{caesar\_shift}       &     F &   F &     Pass &     F &  F &     F &     F &   F &  1   &   0.12  \\
\textbf{is\_prime}      &     F &   Pass &     F &  Pass &  F &     F &     F &   F &  1   &  0.25   \\
\textbf{replace\_from\_another}             &     F &   F &  F &     F &  Pass &     F &     F &   F &   1  &   0.12  \\
\textbf{sum\_digits}        &     Pass &   F &     Pass&     F &  F &  Pass &     F &   F &  1   &  0.37   \\
\textbf{is\_shift\_greater\_than\_len} &  F &   Pass &     F &     F &     F &     F &  Pass &   F &   1  &  0.25   \\
\textbf{get\_floor}              &     F &   F &     F &     Pass &     F &     F &     F &   Pass &  1   &   0.25  \\
\bottomrule
\end{tabular}
    \end{minipage}
    

    \caption{\textbf{Skills Proposed for Questions in $\mathbf{HE_{CF}}$.} Each row represents the name of the sub-skill implemented for a particular question in $HE_{CF}$, with the target question ID forming a diagonal relationship within the table. Upon including the skill as the only element of $V^*$, the constrained GPT-3.5 model was evaluated across the entire dataset (i.e., forming a row), with successful attempts marked as passes. Both Precise Utility (PU) and General Utility (GU) were computed for each sub-skill. (\textbf{top}) Sub-skills proposed by GPT-4 with access to unconstrained, ground truth code for reference. (\textbf{middle}) Sub-skills proposed by GPT-3.5 with no access to ground truth reference code. (\textbf{bottom}) Skills written by a human-expert. Note that the human expert invested considerable time and effort in creating skills that ensured successful passes on the targeted questions.}
    \label{fig:all_skills_table}
\end{figure}

==> Figs/Results/batchfeeding_skills_fig.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width = 0.6\textwidth]{Chapter5/Figs/Section3/hand_selected_skills_results.png}
    \caption{\textbf{Providing sub-skills all-at-once.} The hand-crafted sub-skills are fed to the model all-at-once and evaluated on all 8 questions. Each sub-skill is intended for the question along the diagonal, such as \texttt{is\_prime} for question $82$. (mention q2) The goal is to assess if the model can integrate a single relevant sub-skill when prompted to solve a given coding problem. }
    \label{fig:batch_feeding_skills}
\end{figure}


==> Figs/Results/comparative_fig.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width = 0.9\textwidth]{Figs/Results/human_llm_simple.png}
    \caption{\textbf{Comparing Skills Proposed by Language Models and Humans.} In this comparison, three students from the MLMI cohort, along with GPT-4 and GPT-3.5, were tasked with generating sub-skills for the eight problems within the $HE_{CF}$ dataset. Both the Precise Utility (PU) of the skills and the time required for conception and implementation (i.e., writing the code) were evaluated. The reported averages reveal that human skill proposers, despite their above-average coding ability, produced skills comparable to or even less effective than those proposed by the LMs, while requiring considerably more time. Interestingly, the student who achieved the best results has had extensive experience working with GPT-4 and GPT-3.5, reflecting the influence of familiarity with these models on skill-proposal efficacy.}
    \label{fig:llm_v_human_skills}
\end{figure}

==> Figs/Results/constraining_results_UR.tex <==
\begin{figure}[p]
    \centering
    \includegraphics[width=\textwidth]{Figs/Results/utilisation_rate.png}
    \caption{\textbf{Function Utilisation Rate Across Different Prompt-Parameters and Models.} This figure illustrates the effect of model choice and prompt-configuration on the UR (left y-axis) of functions (replicas) in $V_{rep}$ when answering HumanEval questions. A comparison is made between five specific prompt-configurations and an unconstrained control, for both GPT-3.5 and GPT-4. Overall accuracy on the dataset is represented on the right y-axis, and the goal is to maximize UR without compromising performance. The optimal prompt configuration is identified as $(U,R,C)$, which slightly outperforms $(U,R,C+D)$ while using fewer tokens. In nearly all instances, the models utilise functions from $V_{rep}$ in a majority of code-generations, showing LMs' ability to use unseen functions provided in-context. More details on the prompt configurations can be found in Sec. \ref{sec:prompts_expsetup}.}
    \label{fig:w_replicas}
\end{figure}


==> Figs/Results/constraining_results_fig.tex <==
\begin{figure}[p]
    \centering
    \includegraphics[width=\textwidth]{Figs/Results/non_compliance_rate.png}
    \caption{\textbf{Non-Compliance Rate (NCR) Across Various Prompt Parameters and Models.} We compare the influence of different model choices and prompt configurations on the NCR of a constrained LM when answering HumanEval questions. Five specific prompt configurations are tested alongside an unconstrained control, which serves as a reference for understanding how often invalid functions are used without constraints. Even with the optimal model and configuration, the NCR remains above 50\% of the control's rate, an expected outcome given the restriction of functions from the Python Standard Library, which are frequently encountered during training. A comparison between $(U,NR,C)$ and $(U,R,C)$ configurations further shows that explicitly listing invalid functions enhances compliance. In the best case, GPT-4 only marginally outperforms its predecessor, indicating that preventing models from using highly exposed functions is a more challenging task than encouraging them to use new functions provided in-context. For additional details on the prompt configurations, refer to Sec. \ref{sec:prompts_expsetup}.}



    \label{fig:w_invalids}
\end{figure}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\textwidth]{Chapter5/Figs/Section1/utilisation_rate.png}
%     \caption{\textbf{Evaluating use of replica functions for different prompting methods.} We analyse the percent of completions which call at least one of the custom replica functions. This gives us an idea of how }
%     \label{fig:w_replicas}
% \end{figure}


==> Figs/Results/gpt4_on8_table.tex <==
\begin{figure}
\centering
\begin{tabular}{lllllllll|ll}
\toprule
\textbf{} & \textbf{2} & \textbf{84} & \textbf{89} & \textbf{79} & \textbf{154} & \textbf{110} & \textbf{65} & \textbf{82} & \textbf{PU} & \textbf{GU} \\
\midrule
\textbf{get\_decimal\_part}          &  Pass &   F &     F &     F &     F &     F &     F &   F &   1  &  0   \\
\textbf{sum\_of\_digits}             &     F &   F &     F &     F &     F &     F &     F &   F & 0    &  0   \\
\textbf{join\_list\_to\_string}       &     F &   F &     F &     F &  Pass &     F &     F &   F &  0   &   0.12  \\
\textbf{format\_binary\_string}      &     F &   F &     F &  Pass &  Pass &     F &     F &   F &    1 & 0.25    \\
\textbf{rotate\_string}             &     F &   F &  Pass &     F &  Pass &     F &     F &   F &  1   &  0.25   \\
\textbf{count\_even\_numbers}        &     F &   F &     F &     F &  Pass &  Pass &     F &   F &  1   &   0.25  \\
\textbf{calculate\_effective\_shift} &  Pass &   F &     F &     F &     F &     F &  Pass &   F &  1   &  0.25   \\
\textbf{is\_divisible}              &     F &   F &     F &     F &     F &     F &     F &   F &  0   &  0   \\
\bottomrule
\end{tabular}

  \caption{\textbf{Automated Skills and Their Results on the $\mathbf{HE_{CF}}$ Dataset.} This table presents a detailed examination of the skills, proposed by GPT-4, for all questions within the dataset (question IDs are shown as column headers). Each row represents a skill tailored for a particular question, with the corresponding question ID forming a diagonal relationship within the table. For instance, the skill \textit{get\_decimal\_part} was proposed to address question ID 2. Upon including the skill as the only element of $V^*$, the constrained GPT-3.5 model was evaluated across the entire dataset, with successful attempts marked as passes. Both Precise Utility (PU) and General Utility (GU) were computed for each skill, providing insights into their individual and collective effectiveness. The key takeaway is that although the LM underperforms the human-expert, it can still propose useful skills with less time and effort.}
    \label{fig:gpt4_skills_table}
\end{figure}


==> Figs/Results/gpt_on19_table.tex <==
\begin{figure}
    \centering
\begin{tabular}{llllllllllllllllllll}
\toprule
{} & 111 & 93  & 145 &   135 &   126 &   131 & 108 &   132 & 125 & 119 &   137 & 120 & 140 & 130 & 32  & 129 &   75  & 163 &   91  \\
\midrule
count\_elements                 &   F &   F &   F &     F &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &     F &   F &     F \\
swap\_case\_and\_replace\_vowels   &   F &   F &   F &  Pass &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &     F &   F &     F \\
get\_sum\_of\_digits\_and\_index    &   F &   F &   F &     F &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &     F &   F &     F \\
find\_index                     &   F &   F &   F &  Pass &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &     F &   F &     F \\
check\_duplicates               &   F &   F &   F &     F &  Pass &     F &   F &     F &   F &   F &  Pass &   F &   F &   F &   F &   F &     F &   F &     F \\
multiply\_elements\_in\_list      &   F &   F &   F &     F &     F &  Pass &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &  Pass &   F &     F \\
sum\_of\_signed\_digits           &   F &   F &   F &     F &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &     F &   F &     F \\
check\_nested\_brackets          &   F &   F &   F &     F &     F &     F &   F &  Pass &   F &   F &     F &   F &   F &   F &   F &   F &     F &   F &     F \\
count\_odd\_ord\_lowercase        &   F &   F &   F &     F &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &     F &   F &     F \\
check\_balanced\_parentheses     &   F &   F &   F &     F &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &     F &   F &     F \\
convert\_to\_float               &   F &   F &   F &     F &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &     F &   F &     F \\
get\_top\_k\_elements             &   F &   F &   F &     F &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &     F &   F &     F \\
replace\_consecutive\_chars      &   F &   F &   F &     F &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &  Pass &   F &     F \\
calculate\_tribonacci           &   F &   F &   F &     F &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &     F &   F &     F \\
evaluate\_polynomial            &   F &   F &   F &     F &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &     F &   F &     F \\
get\_min\_neighbor               &   F &   F &   F &  Pass &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &     F &   F &     F \\
prime\_factors                  &   F &   F &   F &     F &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &  Pass &   F &     F \\
generate\_even\_numbers\_in\_range &   F &   F &   F &     F &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &     F &   F &     F \\
split\_into\_sentences           &   F &   F &   F &     F &     F &     F &   F &     F &   F &   F &     F &   F &   F &   F &   F &   F &  Pass &   F &  Pass \\
\bottomrule
\end{tabular}

    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

==> Figs/Results/handfeeding_skills_fig.tex <==
% \begin{figure}[!h]
%     \centering
%     \includegraphics[width = 0.6\textwidth]{Chapter5/Figs/Section3/hand_selected_skills_results.png}
%     \caption{\textbf{Providing sub-skills one-at-a-time vs. All-at-once} The hand-crafted sub-skills are fed to the model one-at-a-time and evaluated on all 8 questions. Each sub-skill is intended for the question along the diagonal, such as \texttt{is\_prime} for question $82$. (mention q2) The goal is to assess if the model can integrate a single relevant sub-skill when prompted to solve a given coding problem. }
%     \label{fig:hand_feeding_skills}
% \end{figure}


% \begin{figure}
%     \centering
% \begin{tabular}{lllllllll}
% \toprule
% {} &   79   & 154  &   89  &   82  &   110 &   84 &   65  & 2  \\
% \midrule
% remove\_bin\_prefix       &  Pass &   F &     F &     F &     F &     F &     F &   F \\
% rotate\_string             &     F &   Pass &     F &     F &     F &     F &     F &   F \\
% caesar\_shift       &     F &   F &     Pass &     F &  F &     F &     F &   F \\
% is\_prime      &     F &   Pass &     F &  Pass &  F &     F &     F &   F \\
% replace\_from\_another             &     F &   F &  F &     F &  Pass &     F &     F &   F \\
% sum\_digits        &     Pass &   F &     Pass&     F &  F &  Pass &     F &   F \\
% is\_shift\_greater\_than\_len &  F &   Pass &     F &     F &     F &     F &  Pass &   F \\
% get\_floor              &     F &   F &     F &     Pass &     F &     F &     F &   Pass \\
% \bottomrule
% \end{tabular}

%     \caption{Hand-written skills}
%     \label{fig:enter-label}
% \end{figure}

\begin{figure}
    \centering
\begin{tabular}{lllllllll|lll}
\toprule
\textbf{} & \textbf{79} & \textbf{154} & \textbf{89} & \textbf{82} & \textbf{110} & \textbf{84} & \textbf{65} & \textbf{2} & \textbf{PU} & \textbf{GU} \\
\midrule
\textbf{remove\_bin\_prefix}       &  Pass &   F &     F &     F &     F &     F &     F &   F &  1   &  0.12   \\
\textbf{rotate\_string}             &     F &   Pass &     F &     F &     F &     F &     F &   F &   1  &  0.12   \\
\textbf{caesar\_shift}       &     F &   F &     Pass &     F &  F &     F &     F &   F &  1   &   0.12  \\
\textbf{is\_prime}      &     F &   Pass &     F &  Pass &  F &     F &     F &   F &  1   &  0.25   \\
\textbf{replace\_from\_another}             &     F &   F &  F &     F &  Pass &     F &     F &   F &   1  &   0.12  \\
\textbf{sum\_digits}        &     Pass &   F &     Pass&     F &  F &  Pass &     F &   F &  1   &  0.37   \\
\textbf{is\_shift\_greater\_than\_len} &  F &   Pass &     F &     F &     F &     F &  Pass &   F &   1  &  0.25   \\
\textbf{get\_floor}              &     F &   F &     F &     Pass &     F &     F &     F &   Pass &  1   &   0.25  \\
\bottomrule
\end{tabular}

    \caption{\textbf{Handwritten Skills and Their Results on the $\mathbf{HE_{CF}}$ Dataset.} This table presents a detailed examination of the skills, manually crafted by a human expert, for all questions within the dataset (question IDs are shown as column headers). Each row represents a skill tailored for a particular question, with the corresponding question ID forming a diagonal relationship within the table. For instance, the skill \textit{sum\_digits} was proposed to address question ID 84. Upon including the skill as the only element of $V^*$, the constrained model was evaluated across the entire dataset, with successful attempts marked as passes. Both Precise Utility (PU) and General Utility (GU) were computed for each skill, providing insights into their individual and collective effectiveness. Note that the human expert invested considerable time and effort in creating skills that ensured successful passes on the targeted questions. The key takeaway is that providing specific skills is an effective way of overcoming failed questions while still adhering to the constraint of using only functions in $F\in V_{rep}$.}
    \label{fig:handwritten_skills_table}
\end{figure}

==> Figs/Results/is_prime.tex <==
\begin{figure}[!p]
\lstset{
  language=Python,
  basicstyle=\ttfamily\scriptsize,
  breaklines=true,
  showstringspaces=false,
  aboveskip=0.2mm,
  belowskip=0mm,
  emph={is_prime(next_prime), is_prime(length), is_prime}, % Emphasize these words
  emphstyle=\bfseries, % Bold the emphasized words
}


% \centering
\begin{minipage}{0.66\textwidth}
\shadowbox{
    \begin{minipage}{\textwidth}

    \begin{center}\textbf{From APPS} \\ 
    \textit{Proposed Skill}
    \end{center} 

    \begin{lstlisting}
def is_prime(n):
    'Checks and returns whether the given number is prime.'
    if n <= 1:
        return False
    if n <= 3:
        return True
    if n % 2 == 0 or n % 3 == 0:
        return False
    i = 5
    while i * i <= n:
        if n % i == 0 or n % (i + 2) == 0:
            return False
        i += 6
    return True 
    \end{lstlisting}
\begin{center}
    \textit{Solution}
    \end{center} 
\begin{lstlisting}
def get_next_prime(n):
    next_prime = n + 1
    while not is_prime(next_prime):
        next_prime += 1
\end{lstlisting}
    \end{minipage}
}
\end{minipage}
\hfill
\begin{minipage}{0.3\textwidth}
    \shadowbox{
        \begin{minipage}{\textwidth}
        
    \begin{center}\textbf{From HumanEval\_82} \\ 
    \textit{Proposed Skill}
    \end{center} 
        \begin{lstlisting}
def is_prime(n): 
    """Check if a number is prime.""" 
    if n < 2: 
        return False 
    for i in range(2, int(n**0.5) + 1): 
        if n % i == 0: 
            return False 
    return True 
\end{lstlisting}
\begin{center}
    \textit{Solution}
    \end{center} 
\begin{lstlisting}
def prime_length(string): 
    length = get_length(string)
    return is_prime(length)
\end{lstlisting}
        \end{minipage}
    }
\end{minipage}

\vspace{1em}
\centering
\begin{minipage}{\textwidth}
    \shadowbox{
        \begin{minipage}{\textwidth}
       \begin{center}\textbf{From HumanEval\_75} \\ 
    \textit{Proposed Skill}
    \end{center} 
\begin{lstlisting}
def is_prime(n): 
    """Check if a number is prime or not.""" 
    if n <= 1: 
        return False 
    if n <= 3: 
        return True 
    if n % 2 == 0 or n % 3 == 0: 
        return False     
    i = 5 
    while i * i <= n: 
        if n % i == 0 or n % (i + 2) == 0: 
            return False 
        i += 6 
    return True
        \end{lstlisting}

        \begin{center}
    \textit{Solution}
    \end{center} 
\begin{lstlisting}
def is_multiply_prime(a):
    factors = prime_factors(a)
    if get_length(factors) == 3:
        return check_if_all_true(apply_func_to_iterable(is_prime, factors))
    return False
\end{lstlisting}

        \end{minipage}
    }
\end{minipage}

\caption{\textbf{Demonstrating Modularity}. This figure highlights the modularity inherent in our method by illustrating how a single skill (\texttt{is\_prime}) was independently proposed (and successfully used) for three distinct questions across two different datasets. This shows that even though skills are proposed to aid only a specific question, they often possess utility that extends to other tasks.}
\label{fig:is_prime}
\end{figure}


==> Figs/Results/num_skills_plot.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width = 0.6\textwidth]{Figs/Results/num_skills_plot_mod.png}
    \caption{\textbf{Impact of $\mathbf{|V^*|}$ on Performance in $\mathbf{HE_{CF}}$}.
    % This figure analyzes the relationship between the number of functions included in $V^*$ and performance on the $HE_{CF}$ dataset, using functions proposed by GPT-4 (blue), GPT-3.5 (orange), and a human expert (red). The details of the proposed functions are provided in Figures \ref{fig:all_skills_table}. The batch of functions marked in purple are the perfect-handwritten skills after being refined by GPT-4. Results for sub-skills proposed by a non-expert human (Adnaan) are presented in green. The black dot on the right bar plot represents the naive expected accuracy when all functions are added ($|V^*| = 8$), matching the average accuracy across all 8 questions when only a single function is included in the constrained model's context when solving the related question. The model is only able to achieve 50\% of its one-at-a-time accuracy when all human-written functions are provided (red bar plot). But when providing all functions generated by GPT-4, the model achieves 120\% of its one-at-a-time accuracy (blue bar plot).
    }
    \label{fig:numskills_plot}
\end{figure}

==> Figs/Results/ur_ncr_combined_fig.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=6cm]{Figs/Results/utilisation_rate.png}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=6cm]{Figs/Results/non_compliance_rate.png}
    \end{minipage}
    \caption{GPT-4 is only evaluated on the top-three prompt configurations to reduce cost..}
    \label{fig:combined_fig}
\end{figure}

% \begin{figure}[!t]
%     \centering
    
%     \begin{minipage}{0.4\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figs/Results/splits_plot.png}
       
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.43\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figs/Results/num_skills_mod.png}
%     \end{minipage}
%     \caption{(right) Impact of \(|V^*|\) on Performance in \(HE_{CF}\); (left) Analyzing Accuracy on the \(HE_{BP,R}\) Dataset Relative to the Size of the Constraint}
%     \label{fig:ablations}
% \end{figure}
% \begin{figure}[p]
%     \centering
%     \begin{subfigure}[b]{0.45\linewidth}
%         \centering
%         \includegraphics[width=6cm]{Figs/Results/utilisation_rate.png}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.45\linewidth}
%         \centering
%         \includegraphics[width=6cm]{Figs/Results/non_compliance_rate.png}
%     \end{subfigure}
%     \caption{Your new caption here.}
%     \label{fig:combined_fig}
% \end{figure}
